On the Hersch-Weinberger inequality in higher dimensions

We investigate a reverse Faber-Krahn type inequality for the Robin Laplacian in a bounded smooth domain $\Omega \subset \mathbb{R}^N$ whose boundary has two connected components. We prove that a concentric spherical shell maximizes the first eigenvalue over a class of such domains under perimeter and volume constraints, and under an additional convexity assumption when $N \geq 3$. This result generalizes to a wider class, and extends to higher dimensions, the inequality of Hersch [20], whose approach was substantially based on a construction of the so-called effectless cut by Weinberger [35], so that we call it the Hersch-Weinberger inequality. Our method is based on the analysis of the gradient flow of the first eigenfunction and several approximation procedures, without relying on the effectless cut itself. The effectless cut being a complicated object related to the attractor of the gradient flow, we describe its most fundamental topological properties. In particular, we show that it does not necessarily have to be a hypersurface.

==> Preamble.tex <==
\usepackage{graphicx}
\usepackage{epstopdf}
\epstopdfsetup{
	suffix=,
}

\usepackage{subcaption}
\captionsetup[subfigure]{labelfont=rm} %% to change fig no from (A) to (a)



%\renewcommand{\thefigure}{\arabic{figure}}
%\renewcommand{\thesubfigure}{\alph{subfigure}}
\usepackage{setspace,mathrsfs,amsthm,amsmath,amssymb,amsfonts,lipsum,appendix,mathtools,cite,tabularx,fontenc}
\usepackage[shortlabels]{enumitem}

\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
	\newenvironment{rep#1}[1]{%
		\def\rep@title{#2 \ref{##1}}%
		\begin{rep@theorem}}%
		{\end{rep@theorem}}}
\makeatother


\newtheorem{theorem}{Theorem}[section]
%\newreptheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{result}[theorem]{Result}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
%\newtheorem{assumption}[theorem]{Assumption}
%\newtheorem*{assumption*}{Assumption}
\newtheorem{assumption}{Assumption}
\renewcommand*{\theassumption}{\Alph{assumption}}

%\numberwithin{equation}{section}


%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{xca}[theorem]{Exercise}
\newtheorem{conjecture}[theorem]{Conjecture}
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}
\usepackage[nointegrals]{wasysym}
\usepackage[misc]{ifsym}
%\usepackage[amsmath,amsthm,thmmarks]{ntheorem}
\usepackage[dvipsnames]{xcolor}
\definecolor{ao}{rgb}{0.0, 0.5, 0.0}
\definecolor{lasallegreen}{rgb}{0.03, 0.47, 0.19}
\usepackage{hyperref}
\hypersetup{
	colorlinks=true,
	linkcolor=blue,
	filecolor=magenta,      
	urlcolor=black,
	citecolor=OrangeRed,
}
\usepackage[margin=1in]{geometry}
%\textwidth6.5in \textheight10in \hoffset-0.25in \voffset0.25in
\renewcommand\baselinestretch{1.4}
\renewcommand{\labelenumii}{\Roman{enumii}}


\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
\newcommand{\md}[1]{\left\vert #1 \right\vert}
\newcommand{\dq}{\coloneqq}
\newcommand{\qd}{\mathrel{={\!\!\mathop:}}}
\newcommand{\RN}{{\mathbb{R}^n}}
\newcommand{\pr}[1]{{#1}^{\prime}}
\newcommand{\al} {\alpha}
\newcommand{\pa} {\partial}
\newcommand{\be} {\beta}
\newcommand{\de} {\delta}
\newcommand{\De} {\Delta}
\newcommand{\Dep} {\Delta_p}
\newcommand{\ga} {\gamma}
\newcommand{\Ga} {\Gamma}
\newcommand{\om} {\omega}
\newcommand{\Om} {\Omega}
\newcommand{\la} {\lambda}
\newcommand{\ep} {\epsilon}
\newcommand{\tht} {\theta}
\newcommand{\La} {\Lambda}
\newcommand{\si} {\sigma}
\newcommand{\Si} {\Sigma}
\newcommand{\Gr} {\nabla}
\newcommand{\lra} {\longrightarrow}
\newcommand{\no} {\nonumber}
\newcommand{\noi} {\noindent}
\newcommand{\SN}{\mathbb{S}^{d-1}}
\newcommand{\HN}[1]{\H^{#1}}
%\newtheorem{rmk}[definition]{Remark}
\newcommand{\dx}{{\,\rm d}x}
\newcommand{\dt}{{\,\rm d}t}
\newcommand{\dr}{{\,\rm d}r}
\newcommand{\ds}{{\,\rm d}s}
\newcommand{\dS}{{\,\rm dS}}
\newcommand{\da}{{\,\rm d}\al}
\newcommand{\dd}{{\,\rm d}\de}
\newcommand{\dsi}{{\,\rm d}\si}
%\newcommand{\T}{I^{-1}(1)\cap W_{\Ga_1}.}
\newcommand{\T}{\theta}
\newcommand{\dsig}{{\,\rm d}\sigma}


\newcommand{\tb}{\textcolor{blue}}
\newcommand{\tbl}{\textcolor{Blue}}
\newcommand{\tr}{\textcolor{red}}
\newcommand{\tg}{\textcolor {green}}
\newcommand{\tv}{\textcolor {violet}}
\def \tor {\textcolor{orange}}

\newcommand{\Omo}{\Om_{\rm{out}}}
\newcommand{\Omi}{\Om_{\rm{in}}}

\newcommand{\Bf}{{\mathbf}}
%\newcommand{\A}{{\mathcal A}}
\renewcommand{\a}{{\mathfrak{a}}}
\newcommand{\cm}{^\mathrm{c}}
\newcommand{\C}{{\mathcal C}}
\newcommand{\E}{{\mathcal E}}
\newcommand{\F}{{\mathcal F}}
\newcommand{\G}{{\mathcal G}}
\newcommand{\M}{{\mathcal M}}
\newcommand{\hs}{\hspace}
\newcommand{\R}{{\mathbb R}}
\newcommand{\N}{{\mathbb N}}
\renewcommand{\P}{{\mathcal P}}
\renewcommand{\O}{{\mathcal O}}
\def\L{{\mathcal L}}
\def\S{{\mathcal S}}
\def\wp{{{W}^{1,p}}(\Om)}
%\usepackage[foot]{amsaddr}

\newcommand{\Omo}{\Om_{\rm{out}}}
\newcommand{\Omi}{\Om_{\rm{in}}}

\newcommand{\Go}{G_{\rm{out}}}
\newcommand{\Gi}{G_{\rm{in}}}

\newcommand{\ho}{h_{\mathrm{out}}}
\newcommand{\hi}{h_{\mathrm{in}}}

\newcommand{\eps} {\varepsilon}
\newcommand{\ra} {\rightarrow}
\newcommand{\embd} {\hookrightarrow}

\newcommand{\wra} {\rightharpoonup}

\newcommand{\wide}[1]{\widetilde{#1}}
\newcommand{\intRn}{\displaystyle \int _{\mathbb{R}^N}}



\def\dx{{\,\rm d}x}
\def\dt{{\,\rm d}t}
\def\dr{{\,\rm d}r}
%\def\ds{{\,\rm d}s}
%\def\dS{{\,\rm dS}}
\def \tb {\textcolor{blue}}
\def \tr {\textcolor{red}}
\def \tg {\textcolor {green}}

\def\Bf{\mathbf}
\def\A{{\mathscr A}}
\def\B{{\mathscr B}}
\def\C{{\mathcal C}}
\def\D{{\mathcal D}}
\def\E{{\mathcal E}}
\def\H{{\mathcal H}}
\def\L{{\mathcal L}}
\def\M{{\mathcal M}}
\def\mo{{\mathcal M}_0(\Om)}
\def\S{{\mathcal S}}
\def\hs{\hspace}
\def\F{{\mathcal F}}

\newcommand{\Ra} {\Rightarrow}


\usepackage[hyperpageref]{backref}
%\usepackage{amsrefs}


\usepackage{orcidlink}

%Just another size of margins

%\usepackage{a4wide}

\setlength{\parskip}{0.4em}

\usepackage{csquotes}

